Forecasting Trajectory and Behavior of Road-Agents Using Spectral Clustering in Graph-LSTMs

We present a novel approach for traffic forecasting in urban traffic scenarios using a combination of spectral graph analysis and deep learning. We predict both the low-level information (future trajectories) as well as the high-level information (road-agent behavior) from the extracted trajectory of each road-agent. Our formulation represents the proximity between the road agents using a weighted dynamic geometric graph (DGG). We use a two-stream graph-LSTM network to perform traffic forecasting using these weighted DGGs. The first stream predicts the spatial coordinates of road-agents, while the second stream predicts whether a road-agent is going to exhibit overspeeding, underspeeding, or neutral behavior by modeling spatial interactions between road-agents. Additionally, we propose a new regularization algorithm based on spectral clustering to reduce the error margin in long-term prediction (3-5 seconds) and improve the accuracy of the predicted trajectories. Moreover, we prove a theoretical upper bound on the regularized prediction error. We evaluate our approach on the Argoverse, Lyft, Apolloscape, and NGSIM datasets and highlight the benefits over prior trajectory prediction methods. In practice, our approach reduces the average prediction error by approximately 75% over prior algorithms and achieves a weighted average accuracy of 91.2% for behavior prediction. Additionally, our spectral regularization improves long-term prediction by up to 70%.

==> tables/infrastructure.tex <==
\begin{table}[h!]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccc} 
\toprule
Device  &  Quantity  & Model & RAM \\
\hline

\multirow{3}{*}{CPU} & \Tstrut 2 & Intel$^{\tiny{\textregistered}}$ Xeon(R) Silver 4208 CPU @ 2.10GHz $\times$ 32 & 64GB\\
           & \Tstrut 2 & Intel$^{\tiny{\textregistered}}$ Xeon(R) Silver 4208 CPU @ 2.10GHz $\times$ 32 & 32GB \\                    
           & \Tstrut 1 & Intel$^{\tiny{\textregistered}}$ Xeon(R) W-2123 CPU @ 3.60GHz $\times$ 8 & 32GB \\
\midrule
\multirow{2}{*}{GPU} &  \Tstrut 5 & GeForce RTX 2080 Ti/PCIe/SSE2 &  12GB \\
                           & \Tstrut 1 & TITAN Xp/PCIe/SSE2 & 12GB \\


% & Linear Regression                &&&&&&&& \\
% \cline{2-8}
% \midrule
% \toprule
%  \Tstrut &  \Bstrut & Overall \\
% \hline
% \multirow{3}{*}{Argoverse} & Guo et al~\cite{guo2019attention} & & & & & \\

% & Linear Regression                &&&&&&&& \\
% \cline{2-8}

% \midrule

% \hline
% \multirow{3}{*}{Argoverse} & Guo et al~\cite{guo2019attention} & & & & & \\

% & Linear Regression                &&&&&&&& \\
% \cline{2-8}
\bottomrule
\end{tabular}
}
\label{tab: infra}
\caption{Infrastructure used for experiments}
\vspace{-5pt}
\end{table}

==> tables/metadata.tex <==
\begin{table}[h]
\centering
% \resizebox{.8\linewidth}{!}{%
\begin{tabular}{lcc} 
\toprule
Dataset & Batch & Avg. Density  \\
\hline

\multirow{3}{*}{Lyft} & Train & \Tstrut 0.80 \\
           & Val & 0.83 \\
           & Test & 0.84 \\                    
\midrule
\multirow{3}{*}{Argoverse} & Train & \Tstrut  0.75 \\
                           & Val & 0.67 \\
                           & Test & 1.67 \\


\midrule                           
\multirow{3}{*}{Apolloscape} & Train & \Tstrut  3.49 \\
                            & Val & 3.50 \\
                            & Test & 2.56 \\                         
            
% & Linear Regression                &&&&&&&& \\
% \cline{2-8}
% \midrule
% \toprule
%  \Tstrut &  \Bstrut & Overall \\
% \hline
% \multirow{3}{*}{Argoverse} & Guo et al~\cite{guo2019attention} & & & & & \\

% & Linear Regression                &&&&&&&& \\
% \cline{2-8}

% \midrule

% \hline
% \multirow{3}{*}{Argoverse} & Guo et al~\cite{guo2019attention} & & & & & \\

% & Linear Regression                &&&&&&&& \\
% \cline{2-8}
\bottomrule
\end{tabular}
% }
\caption{\textbf{Meta-Feature information} for the Lyft Level 5, Apolloscape, and the Argoverse datasets. The average density is reported by measuring the average number of road-agents per frame.}
\label{tab: meta}
% \vspace{-15pt}
\end{table}


% \begin{table*}[h!]
% \caption{Metadata for the Lyft Level 5, Apolloscape, and the Argoverse datasets.}
% \label{tab: accuracy}
% \centering
% \resizebox{.97\linewidth}{!}{%
% \begin{tabular}{lcccccccccccc}
% \toprule[1.1pt]
% \multirow{2}{*}{Dataset}                       &
% \multicolumn{3}{c}{Number of Videos\Tstrut }         &
% \multicolumn{3}{c}{Video Length \Tstrut }         &
% \multicolumn{3}{c}{Number of Vehicles\Tstrut }         &
% \multicolumn{3}{c}{Density \Tstrut }         & \\
% &
% mean \Tstrut & min & max \Bstrut &
% mean & min & max &
% mean & min & max &
% mean & min & max \\
% \midrule
% % \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|=|=|=|}
% Lyft            &  1.163  &  1.242  &  4.423  &  8.640  & 5.031  &  9.882   &  6.66  &  11.27  & 0.262  &  0.270  &  0.010  &  0.01  \\ 
% Argoverse       &  0.871  &  0.884  &  0.635  &  3.091  & 1.039  &  3.079   &  0.930   &  1.850  & 0.244  & 0.243  &  0.005  &  0.005  \\ 
% Apolloscape     &  0.013  &  0.017  &  1.248  &  11.240  & 1.283  &  11.674  &  0.110  &  0.150  & 0.011  &  0.007  &  -  &  - \\ 
% \bottomrule[1.1pt]
% \end{tabular}
% }
% \vspace{-10pt}
% \end{table*}

==> tables/notation.tex <==
\begin{table}
  \caption{Notations used in the paper. }
  \label{tab: notation}
  \centering
  \resizebox{.9\columnwidth}{!}{%
  \begin{tabular}{|c|l|}
  \hline
    Symbol  & Description \\
    \hline
    $n$ & Number of vehicles\\
    $[m]$ & \{1,2,\ldots,m\} \\
    $\vts{\cdot}$ & Number of non-zero elements in a vector or matrix.\\
    $\mc{I}_d$& Set of indices corresponding to non-zero entries in a vector $d$.\\
    $A_\mc{S}$& Set of columns of $A$, indexed by elements of $\mc{S}$.\\
    $\li_t$ & The $i^{\textrm{th}}$ Laplacian matrix in a sequence of sub-degree matrices. \\
    $d = \textrm{dim}\li_t$ & The dimension number of rows (or columns)) of the laplacian matrix .\\
    $\delta$ & A binary vector of length $n$ such that $\vts{\delta} \ll d$ \\
    $U$ & Eigenvector matrix\\
    $\Lambda$ & Diagonal matrix with eigenvalues on the diagonal.\\
    \hline
  \end{tabular}
%   }
  }
%   \vspace{-10pt}
\end{table}


==> tables/protocol.tex <==
\begin{table}[t]
  \caption{\textbf{Behavior Definitions:} Definitions of the different types of road-agent behaviors. $\lambda_1, \lambda_2$ are constant threshold parameters.}
  \label{tab: behavior_protocol}
  \centering
  \resizebox{.5\columnwidth}{!}{
  \begin{tabular}{lc}
  \toprule
    Behavior  & Definition \\
    \midrule
    Overspeeding &  $\theta^{'} > \lambda_1$.\\
    Neutral & $\lambda_2 \leq \theta^{'} \leq \lambda_1$.\\
    Braking & $\theta^{'} < \lambda_2$. \\
    % Weave & $\Delta C > \eta_1$.\\
    % Overtake & $ \eta_2 \leq \Delta C \leq \eta_1$.\\
    \bottomrule
  \end{tabular}
  }
%   }
\vspace{-5pt}
\end{table}


==> tables/streams.tex <==
\begin{table*}[t]
\caption{We compare our approach with state-of-the-art trajectory prediction methods relying on graph-based input structure. We report the average displacement error (ADE) and the final displacement error (FDE) in ADE(\%)/FDE(\%) format.}
\centering
\resizebox{.8\linewidth}{!}{%
\begin{tabular}{ccc}
\toprule[1pt]
Stream 1 & & Stream 2 \\
\midrule
Input: trajectories &  & Adjacency Matrices\\
Output: Trajectories & & Output 1: Adjacency Matrices\\
Use new loss & $\longleftarrow$& Output 2: Spectrum Matrix\\
 &  & \\ 
\bottomrule[1pt]

\end{tabular}
}
% \label{tab: setupA}
% \vspace{-15pt}
\end{table*}

